Diversity's Double-Edged Sword: Analyzing Race's Effect on Remote Pair Programming Interactions

Remote pair programming is widely used in software development, but no research has examined how race affects these interactions. We embarked on this study due to the historical under representation of Black developers in the tech industry, with White developers comprising the majority. Our study involved 24 experienced developers, forming 12 gender-balanced same- and mixed-race pairs. Pairs collaborated on a programming task using the think-aloud method, followed by individual retrospective interviews. Our findings revealed elevated productivity scores for mixed-race pairs, with no differences in code quality between same- and mixed-race pairs. Mixed-race pairs excelled in task distribution, shared decision-making, and role-exchange but encountered communication challenges, discomfort, and anxiety, shedding light on the complexity of diversity dynamics. Our study emphasizes race's impact on remote pair programming and underscores the need for diverse tools and methods to address racial disparities for collaboration.

==> future.tex <==
\section{Future Work}
\textcolor{blue}{A follow-up study with a larger and more diverse sample size could enhance the generalizability of the research findings. Further research could evaluate a self-reported measure regarding participants' engagement with diversity, diversity and inclusion, and perceptions of race and racial differences. Future studies could delve into additional dimensions of individual identity, including gender, sexual orientation, and disability, as these factors intersect with race, potentially shaping pair programming dynamics.}



==> oldresults.tex <==
\section{Results}

%\textcolor{red}{ this is repetition of data analysis section. Maybe move there parts that are not explained properly.
%We analyzed, qualitatively and quantitatively, whether race effects remote pair programming dynamics for same- and mixed-race participant pairs. We coded and performed statistics on the Main Task transcripts, surveys (self-efficacy, pair programming), and retrospective interviews. The code sets we used are described throughout this section. We used participants retrospective interview responses to triangulate our results. }

%In this section, we will provide a comprehensive analysis of each research question and present key findings that encapsulate the main takeaways from our results.

%In this section, we examined each research question and highlighted key findings to takeaway from our results. 

  \begin{table}[]
    \caption{Same-Race (BB) vs. Same-Race (WhWh) vs. Mixed-Race (BWh) Pairs}
    \scalebox{.75}{
    \begin{tabular}{|c||c|cc||cc||cc||c|}
    \hline
    & \textbf{} & \multicolumn{2}{c||}{\textbf{Same-Race (BB)}} & \multicolumn{2}{c||}{\textbf{Same-Race (WhWh)}} & \multicolumn{2}{c||}{\textbf{Mixed-Race (BWh)}} &  \\ \hline
    & Samples & \multicolumn{1}{c|}{Average}  & SD  & \multicolumn{1}{c|}{Average} & SD & \multicolumn{1}{c|}{Average}  & SD  & P-Value \\ \hline
    Productivity  & 4 & \multicolumn{1}{c|}{28} & 12.36 & \multicolumn{1}{c|}{19.25} & 17.75 & \multicolumn{1}{c|}{32.5} & 19.36 & 0.6063  \\ \hline
    Code Quality  & 4 & \multicolumn{1}{c|}{17.5} & 16.77 & \multicolumn{1}{c|}{14} & 9.25  & \multicolumn{1}{c|}{17.5} & 4.33  & 0.7894  \\ \hline
    Self-Efficacy & 8  & \multicolumn{1}{c|}{6.5}  & 7.58  & \multicolumn{1}{c|}{-4.75} & 12.09 & \multicolumn{1}{c|}{1.5}  & 3.51  & \cellcolor{red!40}0.0759  \\ \hline
    \end{tabular}}
    \label{tab:comparing 3 groups prod,cq,self}
\end{table}

\begin{comment}
\begin{table}[]
\caption{Same-race (BB) vs. Same-race (WhWh) vs. Mixed-Race (BWh) Pairs}
\scalebox{.75}{
\begin{tabular}{|c|c|cccc|cc||c|}
\hline
\multirow{2}{*}{} &
   &
  \multicolumn{4}{c|}{\textbf{Same-Race}} &
  \multicolumn{2}{c||}{\textbf{Mixed-Race}} &
   \\ \cline{2-9} 
 &
   &
  \multicolumn{2}{c|}{\textbf{BB}} &
  \multicolumn{2}{c|}{\textbf{WhWh}} &
  \multicolumn{2}{c||}{\textbf{BWh}} &
   \\ \hline
 &
  Samples &
  \multicolumn{1}{c|}{Average} &
  \multicolumn{1}{c|}{SD} &
  \multicolumn{1}{c|}{Average} &
  SD &
  \multicolumn{1}{c|}{Average} &
  SD &
  P-Value \\ \hline
Productivity &
  4 &
  \multicolumn{1}{c|}{28} &
  \multicolumn{1}{c|}{12.36} &
  \multicolumn{1}{c|}{19.25} &
  17.75 &
  \multicolumn{1}{c|}{32.5} &
  19.36 &
  0.6063 \\ \hline
Code Quality &
  4 &
  \multicolumn{1}{c|}{17.5} &
  \multicolumn{1}{c|}{16.77} &
  \multicolumn{1}{c|}{14} &
  9.25 &
  \multicolumn{1}{c|}{17.5} &
  4.33 &
  0.7894 \\ \hline
Self-Efficacy &
  8 &
  \multicolumn{1}{c|}{6.5} &
  \multicolumn{1}{c|}{7.58} &
  \multicolumn{1}{c|}{-4.75} &
  12.09 &
  \multicolumn{1}{c|}{1.5} &
  3.51 & \cellcolor{red!40}0.0759 \\ \hline
\end{tabular}}
\end{table}
\end{comment}

\subsection{RQ1: How does race affect pair programming dynamics in both same-race and mixed-race pairs?} %What effects does race have on same-race and mixed-race pair programming?
%How does pair programming impact productivity, code quality, self-efficacy, and overall experience in same- and mixed-race pairs of programmers.

\textcolor{red}{make sure we call developers and not programmers throughout the paper}

Pair programming is a well-established, agile, software development method that impacts productivity, code quality, self-efficacy, and overall experience of pairs of developers. We analyzed same- and mixed-race participant pairs interactions and evaluated four factors: (1) productivity - how each participant progressed on the task, (2) code quality - accuracy of written code and test, (3) self-efficacy - a participant's belief in their capability to complete the task, (4) overall experience - what participant's gained from pair programming and test-driven development.

For our quantitative analysis, we used the Kruskal-Wallis Rank Sum Test~\cite{ostertagova2014methodology} to compare three groups (4 same-race Black, 4 same-race White, 4 mixed-race participant pairs). Table \ref{tab:comparing 3 groups prod,cq,self} illustrates the average score, standard deviation (SD), and p-value for four pairs across the three groups. For our qualitative analysis, we observed participant's behavior during the task and analyzed interview responses to triangulate our results. 

%For our quantitative analysis, we used the the Wilcoxon Rank Sum test, , to compare two groups (8 same- and 4 mixed-race participant pairs). We chose to use the Wilcoxon Rank Sum test because we had unequal and small sample sizes~\cite{mann1947test}. Table \ref{tab:prod,cq,self} illustrates the average score, standard deviation (SD), and p-value between the same- and mixed-race pairs. We used the Kruskal-Wallis rank sum test to compare three groups (4 same-race Black, 4 same-race White, 4 mixed-race participant pairs). Table \ref{tab:comparing 3 groups prod,cq,self} illustrates the average score, standard deviation (SD), and p-value between three groups~\cite{ostertagova2014methodology}.

%disparities 
%There is a gap in Computer Science literature on whether these benefits extend to same- and mixed-race pairs. 
%Statistical test (Wilcoxon rank-sum, Kruskal-Wallis, average, standard deviation) and open coding were used to quantitatively and qualitatively analyze the relationships between pairs productivity, code quality, self-efficacy, and knowledge transferred.

\subsubsection{Productivity}
Productivity was assessed based on the completion of the task within the 40-minute timeframe. We scored each pair's work out of 100 points, equally weighing the test cases and code quality. An additional 5 bonus points were awarded for optional code contributions by pairs.\textcolor{blue}{The grading criteria are available here~\cite{}.}

%Productivity was determined by how much each participant pair accomplished during the allotted task time frame (40 minutes). We scored every pairs work out of 100 points, with the test cases and code receiving an equal number of points. Also, we included an additional 5 bonus points for optional code written by pairs. 


Pairs predominantly focused on implementing code rather than writing test cases, even though the intended approach was to follow the principles of test-driven development (TDD), where test cases are typically written before code implementation. Participants were more successful in completing the  \verb|vertical| and \verb|horizontal| win code sections. Specifically, five same-race pairs earned points for their work on  \verb|vertical| or \verb|horizontal| win code, while two same-race pairs received points for developing \verb|taking turns| test cases. In contrast, two mixed-race pairs received points for their contributions to  \verb|vertical| \verb|horizontal| and \verb|diagonal| win code sections. It's worth noting that all pairs utilized online resources, such as Stack Overflow, for assistance with Java programming syntax. Additionally, to expedite their progress, pairs frequently copied and pasted existing code segments when adding or creating new methods.

%Pairs mostly progressed through code instead of test cases. Pair were more likely to complete the \verb|vertical| and \verb|horizontal| win code. Five same-race pairs received points for \verb|vertical| or \verb|horizontal| win code. Two same-race pairs received points for creating \verb|taking turns| test cases. Two mixed-race pairs received points for \verb|vertical| \verb|horizontal| and \verb|diagonal| win code. All pairs used online resources (i.e. Stack Overflow) when they were unsure of Java programming syntax. To add to or create new methods, the pairs copied and pasted code. This helped pairs make more progress within the time limit.  

%\textcolor{red}{Implications of this}

%Table \ref{tab:comparing 3 groups prod,cq,self} quantitatively compares the average, standard deviation, and p-value across 3 groups (4 same-race Black, 4 same-race White, 4 mixed-race). Mixed-race pairs had the highest average score (32.5) compared to same-race Black (28) and same-race White (19.25). Mixed-race pairs had the most spread out productivity scores with the highest standard deviation (19.36). We used the Kruskal-Wallis test to compare the productivity scores of the 3 groups~\cite{ostertagova2014methodology}. We found an insignificant difference with a p-value of 0.6063 for $\alpha$=0.05.
\begin{itemize}
\item[] \textbf{Key Findings}
 \begin{itemize}
     \item \textbf{\textit {No significant differences between same- and mixed-race participants pairs:}} 
     \textcolor{red}{say that this was used Kruskal-Wallis test}
     We found an insignificant p-value of 0.6063 for $\alpha$=0.05 (refer to Table \ref{tab:comparing 3 groups prod,cq,self}). Mixed-race pairs had the highest average score (32.5) compared to same-race Black (28), and same-race White (19.25). However, the scores for mixed-race pairs showed a greater standard deviation (19.36), indicating that the results were more dispersed.
     
     \item \textbf{\textit {Same-race participant pairs distributed the task unevenly:}}
    \textcolor{red}{we need numbers here}
     In the same-race participant pairs one partner completed the majority of the task (developing and implementing) alone. \textcolor{red}{Numbers are not clear --may be merge them and use terminology} For example, P2-M2B2 developed for 68\% of the time and implemented for 86\% of the time. His partner, P2-M1B1, developed for 32\% of the time and implemented for 14\% of the time. P2-M2B2 led the development and implementation for the task. %This conveys that one partner was disengaged from the task and that the pairs didn't explicitly discuss pair programming roles. 
     When asked about the partnership P6-M1Wh1 said \textit{“I felt very outclassed that I did not really know what I was doing. He was moving faster than I could, so when I was trying to sit there and kind of understand the logic, he was quickly moving beyond \dots which I'm okay with \dots I prefer to get something done versus [slowing] it down by me, trying to figure everything out \dots he seemed to jump right in and get to it.”} 
     
     \item \textbf{\textit {Same-race pairs, the driver often took the lead in clarifying directions and generating ideas}} \textcolor{red}{add more def and numbers} P6-M2Wh2 was the driver for 96\% of task and spent quadruple the amount of time thinking of ideas compared to his partner. P2-M1B1 talked about not contributing to the task and letting his partner take the lead, \textit{“I just kind of read the room, and you know if my partner hit a roadblock,...maybe I could like offer [a] suggestion or take the wheel”} \textcolor{red}{The example doesn't support the title}
     
     
     %This lack of knowledge transfer implies that same-race participant pairs didn't experience the full benefits of pair programming. 
     
    \item \textbf{\textit {Mixed-race participant pairs distributed the tasks evenly:}}  All the mixed-race participant pairs evenly distributed the work of developing and implementing the code for the task. One partner led in developing (evaluating and selecting best solution) and the other partner led in implementing (identifying actions that support execution of solution) of the code. For example, P9-M2Wh2 developed for 81\% of the time and P9-M1B1 implemented for 93\% of the time. This demonstrates that mixed-race pairs did not switch programming duties and focused on their respective tasks. In the mixed-race pairs, the navigator led in clarifying directions and generating ideas. For example, P12-W2Wh2 was the navigator for 84\% of the task and spent double the amount of time understanding the directions and crafting ideas compared to her partner. P12-W1B1 mentioned this even distribution of the task, \textit{“\dots In [the Main Task] she identified the problems pretty easily and I was [the] person [who] was like, oh yeah, we have to import the array list so everybody has their shrink \dots”} This phenomenon found in mixed-race pairs is in contrast to what we observed from the same-race pairs. \textcolor{red}{Needs graph..or explain the creativity aspects}
    
    %\textcolor{red}{Do we need this as later leadership and role exchange talk about this}
%We observed...
%\textcolor{red}{ we don't need to talk about creativity.} Table \# shows the codeset we used to identify creativity in our study. Figure \# shows…One transferable quality of pair programming is creativity. We used the Osborn-Parnes Creative Problem Solving (CPS) Process to identify distinct creativity tactics used by pairs~/cite{}. CPS has four phases to determine the creativity of an interaction. CPS is used to teach coding skills in computer science classes~\cite{}. The interesting pattern that we saw was how each pair distributed the Develop and Implement code during the Main Task. 
%\textcolor{red}{Just this text but that also more comprehensive}
%In the mixed-race pairs (P3, P4, P5, P7) Develop and Implement was evenly distributed between both participants. P10-M1B1 had 25 instances of Develop (76\% of total Develop code) and P10-M2Wh2 had 30 instances of Implement (79\% of total Implement code).
 
 %one individual did the majority of the task
%In all of the same-race pairs (P1, P2, P6, P8, P9, P10, P11, P12) one person did the majority of the Develop and Implement. For example, P2-M2B2 had 15 instances of Develop which is slightly more than double of what we observed from P2-M1B1 (7 instances). P2-M2B2 had 49 instances of Implement which is more than 6 times what was seen from P2-M1B1 (8 instances). P2-M2B2 led the majority of the Develop/Implement interaction (64 total instances) compared to P2-M1B1 (15 total instances). 

%P2-M1B1 talked about this pattern we found in his interview by mentioning how he took a backseat when his partner was writing code, “...I just kind of read the room, and you know if my partner hit a roadblock, you know maybe I could like offer [a] suggestion or take the wheel…” When asked if he felt included by his partner while solving the Main Task P2-M1B1 expressed that, “...there [were] definitely times when I was kind of, I didn't know honestly what like what [was] going on…” When asked about the partnership P6-M1Wh1 mentioned how \textit{“I think we both had the same general concepts. We just had different ways we would have implemented it, and I think his was probably the more correct advanced method of implementation compared to mine. So I was fine with letting him go with his thing, but it made it where it was kind of hard for me to troubleshoot anything, any issues that [were] being presented because I couldn't quite understand what he was doing with how. So I mean we had one point where I did, you know, ask for clarification…I think we have the same general concepts of what to do his was just better and more advanced than mine.”}

 \end{itemize}
\end{itemize}

\begin{comment}
\begin{itemize}
\item[] \textbf{Key Finding}
 \begin{itemize}
  \item Item 1
  \item Item 2
  \item Item 3
 \end{itemize}
\end{itemize}
\end{comment}

\subsubsection{Code Quality}

We evaluated the quality and completeness of the code produced by both same- and mixed-race participant pairs. Each pair's work was assessed on a scale of 100 points, with correct code accounting for 60 points, and test cases contributing 40 points. Additionally, we allocated 5 bonus points for any optional code written by the pairs. \textcolor{blue}{The grading criteria are available here~\cite{}}. 

%We assessed the quality and completeness of the code produced by same- and mixed-race participant pairs. We scored productivity and code quality independently. We scored every pairs work out of 100 points, with correct code receiving 60 points and test cases receiving 40 points. Also, we included 5 bonus points for optional code written by pairs. 

Pairs primarily earned points for correctly implementing the \verb|swap player| code. In total, four same-race and three mixed-race participant pairs received points for this aspect of their code. However, the creation of accurate test cases proved to be a challenge for most pairs. Participant P6-M1Wh1 acknowledged the impact of his partner's experience on code quality, stating, \textit{``I think we both had the same general concepts; we just had different ways we would have implemented it, and I think his was probably the more correct advanced method of implementation compared to mine.''}


%Pairs received points mostly for \verb|swap player| code. Four same-race and three mixed-race participant pairs received points for correct \verb|swap player| code. Pairs were mostly unsuccessful in creating correct test cases. P6-M1Wh1 mentioned how his partner's experience affected the code quality, \textit{"I think we both had the same general concepts we just had different ways we would have implemented it, and I think his was probably the more correct advanced method of implementation compared to mine."}

%Table \ref{tab:prod,cq,self} demonstrates that  Table \ref{tab:comparing 3 groups prod,cq,self} found that mixed-race pairs and same-race Black pairs had the same average score (17.5) but the mixed-race pairs scores were more approximate (mixed-race SD = 4.33; same-race Black SD = 16.77). We found an insignificant p-value of 0.7894 for $\alpha$=0.05. We found no major differences between same- and mixed-race pairs regarding code quality. However, through our qualitative analysis of participants retrospective interviews, we found that different perspectives and navigator disengagement may have affected code quality during the Main Task.

\begin{itemize}
\item[] \textbf{Key Findings}
 \begin{itemize}
    \item \textbf{\textit {No significant differences between same- and mixed-race participant pairs:}} 
    We used the Kruskal-Wallis test to compare code quality scores across three groups (refer to Table \ref{tab:comparing 3 groups prod,cq,self}). The results showed that mixed-race pairs and same-race Black pairs had the same average score (17.5), but the scores among mixed-race pairs were more dispersed (mixed-race SD = 4.33; same-race Black SD = 16.77). The p-value obtained was 0.7894, which was not statistically significant at the 0.05 alpha level. This suggests that there were no significant differences in code quality between same- and mixed-race pairs.

It's worth noting that mixed-race pairs seemed to rely on their partners' prior programming experience, which could have contributed to their slightly higher scores. When asked about the impact of having a partner from a different racial group on the quality of their code, P10-M1B1 (a mixed-race pair) mentioned, \textit{``I think that the diversity of experience and what that gets you exposed to \dots I would say that like the diversity of thought came from [P10-M2Wh2] experience in industry \dots and coming from someone that's like a new grad \dots I would say that the diversity of age and experience, played a key factor in like differing mindset and knowledge contribution.''}  \textcolor{red}{Methodology says that they were paired for same age experience.}
    %Table \ref{tab:prod,cq,self} compares the code quality scores of same- and mixed-race pairs. We found an insignificant p-value of 0.5858 for $\alpha$=0.05. The mixed-race pairs had a higher average score (17.5) compared to same-race pairs (15.75). Mixed-race pairs had a smaller standard deviation (5), implying that all of the pairs' scores were more similar. 
    %\textcolor{red}{topic sentence...Should start in paragraph about navigator and mixed race..} 
    \item \textbf{\textit {Navigator in mixed-race participant pairs found majority of the bugs in the task:}} it was observed that the navigator tended to identify the majority of coding bugs, which are errors in the code. For three of the mixed-race participant pairs (P3, P4, P5), the navigator tended to find the majority of the bugs in the task. For instance, P9-M2Wh2 detected 17 bugs in the tasks while serving as the navigator 98\% of the time. For the same proportion of time, his partner P9-M1B1, the driver, discovered 5 bugs. In contrast, in all of the same-race participant pairs the driver found majority of the bugs. For example, P11-W1B1 was the driver 100\% of the time and found 31 bugs compared to her partner, P3-W2B2, who was the navigator 100\% of the time and found 2 bugs. The navigator in same-race participant pairs didn't provide feedback on coding errors which possibly affected the quality of code.


 %   Participants in mixed-race pairs made statements like \textit{So what is it saying? We're missing a colon.} and \textit{"Why is it still on X? Shouldn’t be switching back and forth between X and O?"} to identify bugs. 
 \end{itemize}
\end{itemize}

\begin{figure}[h]
\caption{Participants Self-Efficacy}
\centering
\noindent\scalebox{.75}{%
    \begin{tikzpicture}
    \begin{axis} [
    ybar = 2pt,
    x=0.19cm, %distance between bars
    bar width = 4pt, %width of bar
    width=18cm, 
    height=6.5cm,
    %nodes near coords,
    %nodes near coords style={
        %font=\scriptsize,
    %},
    ymin = 12, 
    ymax = 65, 
    xmax=dummy,
    xticklabel style={rotate=45}, %rotate xtick label
    xtick pos=left,
    ytick pos=left,
    symbolic x coords={P1-M1B1, dummy, dummy, P1-M2B2, dummy, dummy, P2-M1B1, dummy, dummy, P2-M2B2, dummy, dummy, P3-W1B1, dummy, dummy, P3-W2B2, dummy, dummy, P4-W1B1, dummy, dummy, P4-W2B2, dummy, dummy, P5-M1Wh1, dummy, dummy, P5-M2Wh2, dummy, dummy, P6-M1Wh1, dummy, dummy, P6-M2Wh2, dummy, dummy, P7-W1Wh1, dummy, dummy, P7-W2Wh2, dummy, dummy, P8-W1Wh1, dummy, dummy, P8-W2Wh2, dummy, dummy, P9-M1B1, dummy, dummy, P9-M2Wh2, dummy, dummy, P10-M1B1, dummy, dummy, P10-M2Wh2, dummy, dummy, P11-W1B1, dummy, dummy, P11-W2Wh2, dummy, dummy, P12-W1B1, dummy, dummy, P12-W2Wh2, dummy},
    xtick=data,
    enlarge y limits=0.045,
    %enlarge y limits = {abs = .08},
    enlarge x limits = {abs=0.38cm}, %distance betwwen first bar and left edge
    tick label style={font=\scriptsize}, 
    xlabel={\hspace{0.2cm} \textbf{Same-Race (BB)} \hspace{2.5cm} \textbf{Same-Race (WhWh)} \hspace{2.5cm} \textbf{Mixed-Race (BWh)}},
    ylabel={Self-Efficacy Scores},
    xlabel style={font=\scriptsize},
    ylabel style={font=\scriptsize},
    legend image code/.code={
        \draw [#1] (0cm,-0.1cm) rectangle (0.2cm,0.1cm); },
    legend style={
        at={(1.009,1)},
        anchor=north west,
        %legend columns=-1,
        draw=none
        font=\scriptsize,
        %legend cell align=left,
    },
    ]
    %Pre
    \addplot[fill=black!40] coordinates {(P1-M1B1, 52) (P1-M2B2, 54) (P2-M1B1, 42) (P2-M2B2, 47) (P3-W1B1, 47) (P3-W2B2, 40) (P4-W1B1, 42) (P4-W2B2, 41) (P5-M1Wh1, 53) (P5-M2Wh2, 48) (P6-M1Wh1, 42) (P6-M2Wh2, 57) (P7-W1Wh1, 47) (P7-W2Wh2, 47) (P8-W1Wh1, 45) (P8-W2Wh2, 53) (P9-M1B1, 57) (P9-M2Wh2, 52) (P10-M1B1, 51) (P10-M2Wh2, 55) (P11-W1B1, 51) (P11-W2Wh2, 56) (P12-W1B1, 46) (P12-W2Wh2, 39)};
    \addlegendentry{Before Task}
    %Post
    \addplot[fill=blue!40] coordinates {(P1-M1B1, 54) (P1-M2B2, 63) (P2-M1B1, 39) (P2-M2B2, 45) (P3-W1B1, 54) (P3-W2B2, 46) (P4-W1B1, 61) (P4-W2B2, 55) (P5-M1Wh1, 56) (P5-M2Wh2, 49) (P6-M1Wh1, 51) (P6-M2Wh2, 57) (P7-W1Wh1, 38) (P7-W2Wh2, 45) (P8-W1Wh1, 13) (P8-W2Wh2, 47) (P9-M1B1, 57) (P9-M2Wh2, 56) (P10-M1B1, 51) (P10-M2Wh2, 58) (P11-W1B1, 54) (P11-W2Wh2, 59) (P12-W1B1, 40) (P12-W2Wh2, 44)};
    \addlegendentry{After Task}
    \end{axis}
    \draw [dashed] (5.23, -0.2) -- (5.23, 5.1);
    \draw [dashed] (9.22, -0.2) -- (9.22, 5.1);
    \draw (2.6,3.5) [fill=none, draw=green] ellipse (0.2 and 0.5);
    \draw (3.2,2.9) [fill=none, draw=green] ellipse (0.2 and 0.5);
    \draw (3.75,3.5) [fill=none, draw=green] ellipse (0.2 and 1);
    \draw (4.35,3.3) [fill=none, draw=green] ellipse (0.2 and 0.8);
    \draw (7.2,2.8) [fill=none, draw=red] ellipse (0.2 and 0.6); %P10
    \draw (7.8,3.15) [fill=none, draw=red] ellipse (0.2 and 0.3); %P10
    \draw (8.44,1.65) [fill=none, draw=red] ellipse (0.2 and 1.45); %P11
    \draw (8.95,3.5) [fill=none, draw=red] ellipse (0.2 and 0.4); %P11
    \draw (9.48,4) [fill=none] ellipse (0.2 and 0.2); %P5
    \draw (10.05,3.75) [fill=none, draw=green] ellipse (0.2 and 0.4); %P5
    \draw (10.65,3.5) [fill=none] ellipse (0.2 and 0.2); %P7
    \draw (11.2,3.9) [fill=none, draw=green] ellipse (0.2 and 0.4); %P7
    \end{tikzpicture}%
    }
\label{fig:self efficacy}
\end{figure}

\subsubsection{Self-Efficacy}
Figure \ref{fig:self efficacy} displays the self-efficacy scores for each participant, where self-efficacy represents the participants' belief in their own ability to succeed. One notable effect of pair programming is its positive impact on participant morale \cite{Nosek1998}. To quantify this impact, we assessed self-efficacy using a 7-point Likert scale administered through surveys conducted at both the beginning and end of the task. It's important to note that participants' self-efficacy may have been influenced by their interactions with their programming partner. \textcolor{blue}{The surveys are available here~\cite{}.}


%We measured self-efficacy quantitatively, using a 7-point Likert scale through surveys at the beginning and end of the task, as it may have got influenced by interactions with their partner. \textcolor{blue}{The surveys are available here~\cite{}.}

\textcolor{red}{ This paragraph contents are good but may need to go somewhere else?}
Participants explained that their lack of programming and Java syntax knowledge was the cause of their decreased self-efficacy. Participants were reluctant to take the driver role at the beginning of the task due to lower self-efficacy levels. When asked about how they picked their roles P3-W1B1 said, \textit{"I knew going in I wasn't super confident with Java...I haven't [done Java] in a long time, so I think because we're both just not super confident in our Java skills it kind of left a little bit of hesitancy of who was gonna take the wheel."}

\begin{itemize}
\item[] \textbf{Key Findings}
 \begin{itemize}
    \item \textbf{\textit {Slightly significant differences between same- and mixed-race participant pairs:}} 
We conducted a comparison of self-efficacy scores by analyzing the differences between participants' self-reported self-efficacy levels before and after the task. Specifically, we compared the self-efficacy score differences for three groups: same-race Black, same-race White, and mixed-race participant pairs. The results of this comparison are summarized in Table \ref{tab:comparing 3 groups prod,cq,self}. Using  Kruskal-Wallis, we found a slightly significant p-value of 0.0759 for $\alpha$=0.05. We used the Wilcoxon Rank Sum Test~\cite{mann1947test} to compare 8 scores across a combination of two groups: (1) same-race Black $\rightarrow$ same-race White, (2) same-race Black $\rightarrow$ mixed-race, (3) same-race White $\rightarrow$ mixed-race. We found insignificant p-values of (1) 0.1829, (2) 0.123, (3) 0.2041 for $\alpha$=0.05 for all combinations. \textcolor{blue}{no discussion on averages as in Productiving and code quality}

    
%We compared 8 sample self-efficacy scores (difference between before and after self-reported self-efficacy) for same-race Black, same-race White, and mixed-race participant pairs (refer to Table \ref{tab:comparing 3 groups prod,cq,self}).  We found a slightly significant p-value of 0.0759 for $\alpha$=0.05. We used the Wilcoxon Rank Sum Test~\cite{mann1947test} to compare 8 scores across a combination of two groups: (1) same-race Black $\rightarrow$ same-race White, (2) same-race Black $\rightarrow$ mixed-race, (3) same-race White $\rightarrow$ mixed-race. We found insignificant p-values of (1) 0.1829, (2) 0.123, (3) 0.2041 for $\alpha$=0.05 for all combinations.


    
    %\textcolor{red}{give numbers--p-value}
    \item \textbf{\textit {Same-race Black participant pairs self-efficacy increased while same-race White participant pairs self-efficacy decreased:}} Same-race Black pairs had the highest average self-efficacy (6.5) which could be from participants high levels of comfort. Same-race White pairs had the lowest average self-efficacy (-4.75). Both same-race Black woman pairs had a large increase in average self-efficacy (P6: +6.5, P12: +16.5). For example, P4-W1B1 increased by 19 and P4-W2B2 increased by 14 which is the highest self-efficacy increase amongst all the pairs. All four participants attributed their increase in self-efficacy to having a natural feeling/connection, high comfort levels, and feeling involved by their partner. P3-W1B1 mentioned her reasoning for a lower confidence level at the beginning of the study, \textit{“I think we definitely would have benefited if we had a little bit more confidence, I think, in our skill set. I think we both kind of doubted ourselves a little bit. I know I did initially because I tend to not want to over compensate.”} 
    
    Both same-race White woman pairs average self-efficacy decreased (P10: -5.5, P11: -19). For example, P7-W1Wh1 decreased by 9 and P7-W2Wh2 decreased by 2. Participants attributed their decrease in self-efficacy to difficulty with Java programming syntax and making little progress in the task. When asked about self-efficacy P8-W1Wh1f said, \textit{"That ended up really hurting my confidence, because I felt that I was performing poorly \dots"} Our findings contradict pair programming studies that reported woman having increased self-efficacy when working together~\cite{Kuttal2019, choi2013evaluating, choi2015comparative, mcdowell2006pair, ying2019their}.

    \item \textbf{\textit {No major patterns across mixed-race participant pairs self-efficacy:}} The mixed-race pairs average self-efficacy scores (1.5) were the most approximate (SD = 3.51). The main pattern we observed was between the mixed-race man participant pairs. The Black male participants' self-efficacy remained constant (P9-M1B1: 0, P10-M1B1: 0) whereas the White male participants' self-efficacy increased (P9-M2Wh2: +4, P10-M2Wh2: +3). There was no pattern across the mixed-race woman participant pairs. We used the Wilcoxon Rank Sum Test to compare 4 samples across two groups (Black and White mixed-race participants). We found a insignificant p-value of 0.1814 for $\alpha$=0.05. 
 \end{itemize}
\end{itemize}

%Large increase in same-race Black woman pairs, Decrease in same-race White woman pairs self-efficacy: 

\begin{tcolorbox}[width=\textwidth,
    colback={black!10},
    %title={RQ3 - Diversity's Double-Edged Sword},
    %colbacktitle=blue!40,
    %coltitle=black
    ]
    \begin{center}
        Diversity had a positive impact on pair programming due to equal task distribution and quality of code.
    \end{center}
\end{tcolorbox}

\subsection{RQ2: How does race influence collaboration dynamics among pair programmers?}

To understand the key dynamics and factors that influence collaboration between developers of the same race and those of different races, and how these dynamics impact software development outcomes, we analyzed the study data and interviews.

\begin{table}[h]
    \centering
    \caption{Leadership Styles Codes}
    \scalebox{.75}{
    \begin{tabular}{|p{2.2cm}|p{5.5cm}|p{11.5cm}|}
        \hline
        \textbf{Codes} & \textbf{Definitions} & \textbf{Our Study Examples}\\
        \hline
        \hlc[orange!40]{Authoritative} & When P1 dominates the interaction/makes decisions alone and P2 follows/doesn't contribute any input & \textit{P1: I'm gonna just add this other thing before time runs out, for if the board is full, then we just end the game.} \\
        \hline
        \hlc[orange!40]{Democratic} & When P1 shares the decisions with the other P2 or encourages P2 to take initiative & \textit{P1: I was thinking we can update it in the place mark, or we can update it at the end of the checkInput. \hfill \break P2: Well, because the checkInput is checking for a single player, though I think it's really it should be flipping wherever checkInput is called right? } \\
        \hline
        Laissez-faire & When P1 says do what you think is right and gives all decision making to P2 & \textit{P1: I see. Okay, yeah, do it. You do your idea, then. Great. Sorry. } \\
        \hline
        \hlc[orange!40]{Paternalistic}& When P1 teaches/instructs P2 or leads in a ‘fatherly/motherly’ way & \textit{P2: So explain to me the difference between game dot and this dot. \hfill \break P1: So game dot is referencing, if you look at the main Java file on line 5, that's where we're creating the variable game, and then you can call methods from that and you can reference that game [or] object you could say by calling it game. If I wanted to, I could create another one here and call it game2 so then I've created 2 tic-tac-toe games\dots} \\
        \hline
        Transformational & When P1 changes, transforms, or redirects thoughts and P2 starts thinking the same way as P1 & \textit{P1: Before we put all of them in there let's see if one if statement works. \hfill \break  P2: Yeah, I was about to say that next just test it right now [so] we can see if the initial works. Yeah.} \\
        \hline
    \end{tabular}}
    \label{tab:leadership codeset}
\end{table}

\begin{figure}[h]
\caption{Percentage of Time Participants Spent Using Each Leadership Style }
\centering
\noindent\scalebox{.75}{%
    \begin{tikzpicture}
        \begin{axis}[
        name=MyAxis,
        xbar stacked,
        width=10cm, 
        height=10cm, 
        bar width=5.5pt,
        enlarge y limits=0.045,
        xtick pos=left,
        ytick pos=left,
        xlabel={Overall Interaction},
        ylabel={Mixed-Race (BWh) \hspace{1cm} Same-Race (BB)  
        \hspace{1cm} Same-Race (WhWh)},
        xmin=0, 
        xmax=100,
        legend pos=outer north east,
        legend style={font=\footnotesize},
        tick label style={font=\footnotesize}, 
        %ylabel={\hspace{1.7cm} \textbf{Same-Race} \hspace{2.7cm} \textbf{Mixed-Race}},
        ylabel style={font=\footnotesize},
        xticklabel={$\pgfmathprintnumber{\tick}\%$},
        symbolic y coords={P9-M1B1, P9-M2Wh2, dummy, P10-M1B1, P10-M2Wh2, dummy, P11-W1B1, P11-W2Wh2, dummy, P12-W1B1, P12-W2Wh2, dummy, P1-M1B1, P1-M2B2, dummy, P2-M1B1, P2-M2B2, dummy, P3-W1B1, P3-W2B2, dummy, P4-W1B1, P4-W2B2, dummy, P5-M1Wh1, P5-M2Wh2, dummy, P6-M1Wh1, P6-M2Wh2, dummy, P7-W1Wh1, P7-W2Wh2, dummy, P8-W1Wh1, P8-W2Wh2},
        ytick=data,
        ]
        %A
        \addplot[color=black, fill=green!40]  coordinates {(47.5,P9-M1B1) (34.55,P9-M2Wh2) (41.38,P10-M1B1) (51.72,P10-M2Wh2) (31.11,P11-W1B1) (35.71,P11-W2Wh2) (40.68,P12-W1B1) (41.38,P12-W2Wh2) (69.74,P1-M1B1) (50,P1-M2B2) (81.25,P2-M1B1) (81.82,P2-M2B2) (60.47,P3-W1B1) (45.61,P3-W2B2) (51.47,P4-W1B1) (22.92,P4-W2B2) (53.52,P5-M1Wh1) (40,P5-M2Wh2) (27.27,P6-M1Wh1) (55.77,P6-M2Wh2) (22.5,P7-W1Wh1) (36.54,P7-W2Wh2) (16.67,P8-W1Wh1) (31.82,P8-W2Wh2)};
        %D
        \addplot[color=black, fill=blue!40]  coordinates {(42.5,P9-M1B1) (34.55,P9-M2Wh2) (51.72,P10-M1B1) (41.38,P10-M2Wh2) (64.44,P11-W1B1) (61.9,P11-W2Wh2) (49.15,P12-W1B1) (48.28,P12-W2Wh2) (25,P1-M1B1) (36,P1-M2B2) (12.5,P2-M1B1) (6.06,P2-M2B2) (24.42,P3-W1B1) (36.84,P3-W2B2) (30.88,P4-W1B1) (45.83,P4-W2B2) (11.27,P5-M1Wh1) (20,P5-M2Wh2) (59.09,P6-M1Wh1) (30.77,P6-M2Wh2) (37.50,P7-W1Wh1) (30.77,P7-W2Wh2) (50,P8-W1Wh1) (15.91,P8-W2Wh2)};
        %L
        \addplot[color=black, fill=black!40]  coordinates {(0,P9-M1B1) (9.09,P9-M2Wh2) (3.45,P10-M1B1) (3.45,P10-M2Wh2) (0,P11-W1B1) (0,P11-W2Wh2) (1.69,P12-W1B1) (0,P12-W2Wh2) (0,P1-M1B1) (4,P1-M2B2) (0,P2-M1B1) (0,P2-M2B2) (1.16,P3-W1B1) (0,P3-W2B2) (0,P4-W1B1) (4.17,P4-W2B2) (0,P5-M1Wh1) (0,P5-M2Wh2) (0,P6-M1Wh1) (0,P6-M2Wh2) (0,P7-W1Wh1) (0,P7-W2Wh2) (0,P8-W1Wh1) (0,P8-W2Wh2)};
        %P
        \addplot[color=black, fill=red!40]  coordinates {(5,P9-M1B1) (16.36,P9-M2Wh2) (0,P10-M1B1) (0,P10-M2Wh2) (2.22,P11-W1B1) (0,P11-W2Wh2) (3.39,P12-W1B1) (3.45,P12-W2Wh2) (1.32,P1-M1B1) (2,P1-M2B2) (3.13,P2-M1B1) (3.03,P2-M2B2) (12.79,P3-W1B1) (15.79,P3-W2B2) (14.71,P4-W1B1) (22.92,P4-W2B2) (29.58,P5-M1Wh1) (23.33,P5-M2Wh2) (13.64,P6-M1Wh1) (13.46,P6-M2Wh2) (30,P7-W1Wh1) (26.92,P7-W2Wh2) (33.33,P8-W1Wh1) (52.27,P8-W2Wh2)};
        %T
        \addplot[color=black, fill=orange!40]  coordinates {(5,P9-M1B1) (5.45,P9-M2Wh2) (3.45,P10-M1B1) (3.45,P10-M2Wh2) (2.22,P11-W1B1) (2.38,P11-W2Wh2) (5.08,P12-W1B1) (6.9,P12-W2Wh2) (3.95,P1-M1B1) (8,P1-M2B2) (3.13,P2-M1B1) (9.09,P2-M2B2) (1.16,P3-W1B1) (1.75,P3-W2B2) (2.94,P4-W1B1) (4.17,P4-W2B2) (5.63,P5-M1Wh1) (16.67,P5-M2Wh2) (0,P6-M1Wh1) (0,P6-M2Wh2) (10,P7-W1Wh1) (5.77,P7-W2Wh2) (0,P8-W1Wh1) (0,P8-W2Wh2)};
        \legend{\strut Authoritative, \strut Democratic, \strut Laissez-faire, \strut Paternalistic, \strut Transformational}
        \end{axis}
    \draw [dashed] (-2,2.85) -- (9.5,2.85);
    \draw [dashed] (-2,5.55) -- (9.5,5.55);
    \end{tikzpicture}%
}    
\label{fig:leadership figure}
\end{figure}

\subsubsection{Effect of Leadership Style}
Table ~\ref{tab:leadership codeset} is the code set we used to label leadership styles which is inspired by various works~\cite{cuadrado2012gender, Kuttal2019, adeliyi2021investigating, bass1996transformational}. Figure ~\ref{fig:leadership figure} illustrates the percentage of time each participant spent using a certain leadership style. Leadership style is an important aspect to consider during remote pair programming. Management research has explored how race impacts self-perception, how others perceive and treat you, and evaluations all of which can influence an individual's leadership style~\cite{ospina2009critical, case1997african, lomotey1993african}. We found that mixed-race participant pairs showed slightly greater democratic style. In same-race participant pairs, one partner displayed a mostly authoritative style. The same-race White and same-race Black woman participant pairs displayed a large amount of the paternalistic style. We will discuss the authoritative, democratic, and paternalistic styles seen at high amounts throughout the pairs interactions.


\begin{itemize}
\item[] \textbf{Key Findings}
 \begin{itemize}
    \item \textbf{\textit {Same-race participant pairs had a solo decision-making partner:}} All of the same-race participant pairs displayed similar leadership behaviors toward one another. For the majority of the interaction, one participant displayed an authoritative style more than the other partner. The authoritative partner made majority of the coding decisions alone during the task. For example, in P1 (same-race pair), P1-M1B1 was authoritative 20\% more than P1-M2B2 during the interaction. Another example, in P9 (same-race pair) P6-M2Wh2 was about 30\% more authoritative than P6-M1Wh1. In the task, P6-M2Wh2 said, \textit{“I'm just gonna do this [add a variable], so that I don't have to use self [keyword] and hopefully, that does it”.} The dialogue is an example of an authoritative partner making code design decisions alone. In the same-race participant pairs, the authoritative participant took control over the task implicitly or explicitly more than the other participant. P5-M2Wh2 talked about his implicit task management and leadership style during the task, \textit{“Maybe I was a little more eager to jump on it and just start looking around\dots but I definitely I think I started out just jumping around, looking around, reading and I think he [P5-M2Wh2] kind of filled into that navigator role\dots”}
    \item \textbf{\textit {Mixed-race participant pairs shared decision-making:}} Mixed-race participant pairs spent roughly an equal percentage of the interaction employing the authoritative and democratic style but were slightly more democratic. For example, both participants in P12 (mixed-race pair) spent approximately an equal amount of time using both styles (authoritative - 41\%, democratic - 48\%). The mixed-race pairs were largely authoritative during the beginning and end of the task due to the pressure of trying to finish before the time limit. In general, the more democratic pairs (mixed-race pairs) were more successful as far as productivity and code quality. Partners within mixed-race pairings transitioned between leadership styles by explicitly releasing control of the task. We observed that man and woman mixed-race pairs transitioned between leadership styles using different patterns. For example, P5 and P7 (mixed-race men) were democratic when discussing ideas/directions and authoritative when developing code. In contrast, P11 and P12 (mixed-race women) were authoritative in the beginning when coming up with ideas, deciding which problem to solve first and shifted to a democratic style when writing code. P11-W2Wh2 verified the democratic trends we saw when asked about how the partnership felt, \textit{"I personally felt like it was pretty democratic. I feel like since we're both like a little bit older students, it's a lot easier to kind of let the other person take the reins because we there's some like maturity. They're not needing to constantly be like the person speaking or like doing all the things. Overall, I felt like it was pretty democratic."} Management research studies discovered that mixed-race entrepreneurial teams shared decisions more democratically, in the workplace, while performing tasks~\cite{bass1990bass, bass2008handbook}.
    \item \textbf{\textit {Same-race White (irrespective of gender) and Black women participant pairs educated each other during the task:}} The same-race White pairs showed a large amount of the paternalistic style on average (P8 - 26\%, P9 - 14\%, P10 - 28\%, P11 - 43\%). We observed a high amount of the paternalistic style in the same-race Black woman pairs on average (P6 - 15\%, P12 - 19\%). The pairs tended to use this style when instructing or helping their partner on Java programming syntax. For example, P5-M1Wh1 instructed P5-M2Wh2 on writing the method to switch players between X and O for the task, \textit{“So leave that method, the getPlayer one, leave that the way it is, create another method right below it\dots perfect, and then go ahead and put a parameter in there, so setPlayer and in those parentheses do, like char\dots there you go, and then just do\dots lowercase c-h-a-r, maybe newMark\dots I think it's just one [equal sign]\dots”} while P5-M2Wh2 followed the directions. P6-M2Wh2 confirmed the style we observed in the interview, \textit{"If you're coaching them through syntactical things sometimes it's like here's simpler ways of writing what you wrote or hey you're missing the class name, or you're missing the new keyword\dots you find yourself needing to catch some of those things just because they're stuck\dots"} \textcolor{blue}{find literature}
 \end{itemize}
\end{itemize}

\begin{comment}
\begin{figure}[!h]
    \centering
    \caption{Interruptions Overtime}
    \noindent\scalebox{.75}{%
    \includegraphics[width=0.75\textwidth]{Figures/interruption.png}}
    \label{interruptions}
    \vspace{-18pt}
\end{figure}
\end{comment}

\begin{comment}
\subsubsection{Effect of Partners' Interruptions}
Figure \ref{interruptions} shows the same- and mixed-race participant pairs interruptions overtime. An individual starting up some sort of intervention while another person's turn is still in progress is known as an interruption. Interruptions are correlated with interpersonal control~\cite{}, sociability~\cite{}, interest~\cite{}, and participation in the task~\cite{}. During the task, participants interrupted their partner to help them with Java syntax and generating ideas. Interruptions led to more correct code but slowed pairs progress because they diverted a partners' attention.
\end{comment}

\begin{comment}
BB
P1: 11  +
P2: 2
P6: 4
P12: 6

WhWh
P8: 7
P9: 19 +
P10: 14 +
P11: 4

BWh
P5: 29  +
P7: 6
P3: 6
P4: 11 +
\end{comment}

\begin{comment}
\begin{itemize}
\item[] \textbf{Key Finding\textcolor{blue}{s}}
 \begin{itemize}
    \item \textbf{\textit {\textcolor{blue}{Mixed-race participant pairs felt more interrupted by their partner during the task:}}} Three partners in mixed-race participant pairs felt more interrupted during the task. 
    \item \textbf{\textit {}}
 \end{itemize}
\end{itemize}
\end{comment}

\pgfplotstableread[col sep=&, header=true]{
Question&v1&v2&v3
Q1&4.125 & 4.125&4
Q2&4.125 &4 &4.25
Q3& 4&3.875 &3.875
Q4&4.375 &4.5 &4.625
Q5&4.5 &4.25 &4.375
Q6&4.5 &3.75 &3.25
Q7&4.75 &3.625 &3.75
Q8& 2.125&2.875 &2.5
Q9&1.625 &2.5 &1.875
Q10&2.25 & 2.25&1.875
Q11&2.125 &3 &2
Q12& 2.25&3.25 &2.25
Q13& 2.25& 3.625&2.5
Q14& 2.125&2.75 &2
Q15& 3.875&3.375 &3.125
Q16&4.25 &3.75 &3.5
Q17&4.25 &3.5 &3.625
Q18&4.125 & 3.5&3.5
Q19&4.5 &4.25 &4.25
}\ppdata

\begin{figure}[h]
\caption{Pair Programming Preferences Questionnaire}
\vspace{5pt}
\begin{minipage}[c]{8.5cm}
\centering
%\noindent\scalebox{.75}{%
    \begin{tikzpicture}
        \begin{axis}[
        xtick=data,
        xticklabels from table={\ppdata}{Question},  
        width=8cm, 
        height=8cm,
        bar width=10mm, y=6mm,
        xtick pos=left,
        ytick pos=left,
        enlarge x limits = {abs=0.2cm},
        xlabel={Survey Questions},
        xlabel style={font=\scriptsize},
        ylabel style={font=\scriptsize},
        ylabel={Average Scores},
        ytick={0,1,2,3,4,5,6},
        ymin=0,
        ymax=7,
        xticklabel style={rotate=45, font=\scriptsize},
        yticklabel style={font=\scriptsize},
        %xmin=0, 
        %xmax=100,
        legend pos=inner north east,
        legend style={font=\tiny},
        tick label style={font=\scriptsize},
        nodes near coords align={vertical},
        ]
        %BB
        \addplot [blue!40,mark=*]  table [ybar, y=v1, x expr=\coordindex,] {\ppdata};
        %WhWh
        \addplot [red!40,mark=diamond*] table [y=v2, x expr=\coordindex] {\ppdata};
        %BWh
        \addplot [green!40,mark=square*] table [y=v3, x expr=\coordindex] {\ppdata};
        \legend{\strut Same-Race (BB), \strut Same-Race (WhWh), \strut Mixed-Race (BWh)}
        \end{axis}
    \end{tikzpicture}
    %}
    \end{minipage}%
    \begin{minipage}[c]{7cm\textwidth}
      \scriptsize
      \textbf{1 } Strongly Disagree / Very Low / Very Poor / Very Dissatisfied \\
      \textbf{2 } Disagree / Low / Poor / Dissatisfied \\
      \textbf{3 } Neutral \\
      \textbf{4 } Agree / High / Well / Satisfied \\
      \textbf{5 } Strongly Agree / Very High / Very Well / Very Satisfied \\
      \rule{170pt}{0.3} \\
      Pair Programming with Test-Driven Development produced \\
      \textbf{1 + } Higher quality code \hspace{24.5pt} \textbf{8 - } Inefficient use of time\\
      \textbf{2 + } Constant code review  \hspace{20pt} \textbf{9 - } Personality clashes \\
      \textbf{3 + } Better design \hspace{40pt} \textbf{10 - } Disagreements\\
      \textbf{4 + } Can learn from partner  \hspace{16pt} \textbf{11 - } Skill level differences \\
      \textbf{5 + } Better testing \& debugging \hspace{6.5pt} \textbf{12 - } Personal style differences\\
      \textbf{6 + } Improved creativity \hspace{24.5pt} \textbf{13 - } Distracting interruptions \\
      \textbf{7 + } Improved morale \hspace{31pt} \textbf{14 - } Communication issues\\
      \rule{170pt}{0.3} \\
      My \dots with Pair Programming with Test-Driven Development \\
      \textbf{15 + } Confidence in solution \hspace{14pt} \textbf{16 + } Enjoyment of technique\\
      \rule{170pt}{0.3} \\
      Pair Programming with Test-Driven Development works for \\
      \textbf{17 + } me \hspace{10pt} \textbf{18 + } my partner \hspace{10pt} \textbf{19 + } interactions with partner \\ \\ \\
   \end{minipage}
\label{fig: pp post study}
\end{figure}


\subsubsection{Overall Experience} We measured participants overall experience with pair programming and test-driven development. We collected participants pair programming and test-driven development preferences individually using a questionnaire adapted from Kuttal et. al~\cite{Kuttal2021}. These responses helped to triangulate our findings in RQ1. \textcolor{blue}{The questionnaire is available here~\cite{}.} 

Figure \ref{fig: pp post study} shows the average response for same-race Black, same-race White, mixed-race participant pairs per question. Each trend line represents a group and the points are the average response scores for each question. We asked participants 19 questions about their pair programming and test-driven development preferences. Participants rated each question using values 1 - 5 with 1 as the lowest response (Strongly Disagree / Very Low / Very Poor / Very Dissatisfied) and 5 as the highest response (Strongly Agree / Very High / Very Well / Very Satisfied). Whether a higher or lower value is preferred is indicated beside the question numbers with a (+) or (-) sign.

\begin{itemize}
\item[] \textbf{Key Findings}
 \begin{itemize}
    %Learned new techniques (TDD) from partner
    \item \textbf{\textit {Significant differences between same- and mixed-race participant pairs preferences:}} We used the Kruskal-Wallis test to compare 8 participants pair programming preferences for three groups (same-race Black, same-race White, mixed-race). We found insignificant p-values for majority of the questions. We found a significant p-value of 0.03491 for $\alpha$=0.05 for question 6, which was "pair programming with test-driven development produced improved creativity". We found a significant p-value of 0.0323 for $\alpha$=0.05 for question 7, which was "pair programming with test-driven development produced improved morale". These significant p-values indicates that the three groups had differing opinions on question 6 and 7. For questions 1-5, all three groups favorably ranked pair programming.
    %showed more confidence in their morale
    \item \textbf{\textit {Same-race Black participant pairs preferred pair programming:}} The pair programming questionnaire results reinforced our quantitative self-efficacy results for Black participant's. The same-race Black participant pairs preferred pair programming with test driven development (refer to Figure \ref{fig: pp post study}). The same-race Black participants (blue, dotted trend line) had the highest average scores for questions 6 - "improved creativity", 7 - "improved morale", 15 - "confidence in solution", 16 - "enjoyment of technique", 17 - "me", 18 "my partner", and 19 "interactions with partner". These questions preferred higher values because they were benefits of pair programming with test-driven development. Same-race Black participants had the lowest average scores for questions 8 - "inefficient use of time" and 9 - "personality clashes" which preferred lower values. P3-W2B2 mentioned that she prefers pair programming, \textit{“\dots sometimes 2 heads are better than one [when you] look at something\dots somebody else can look at it for a minute and automatically see the error\dots”} Black participants enjoyed pair programming which increased their self-efficacy and morale in completing the task.
    \item \textbf{\textit{Same-race White participant pairs preferred solo programming:}} The pair programming questionnaire results reinforced our quantitative self-efficacy results for White participant's. The same-race White participant pairs preferred to work alone to solve programming problems (refer to Figure \ref{fig: pp post study}). The same-race White participants (red, diamond trend line) had the highest average scores for questions 8 - "inefficient use of time", 9 - "personality clashes", 11 - "skill level differences", 12 - "personal style differences", 13 - "distracting interruptions", and 14 - "communication issues". These questions preferred lower values because they were downsides of pair programming with test-driven development. P5-M2Wh2 talked about his preference for solo programming because of skill level differences, \textit{"If I don't know this stuff and I'm trying to learn while we're trying to actually get work done or vice versa, trying to get someone else caught up that can be kind of detrimental sometimes. Where if you were just working by yourself, you could just knock it out [but instead] you're getting dragged down, and vice versa, you can also be the person that's dragging someone else down. Then you're feeling bad because some people do, unfortunately, show their frustrations when you're not [on] the same level as they are, and then working with someone that's getting frustrated with you that's not fun. I would rather work by myself\dots"} White participants ranked pair programming unfavorably which negatively impacted their self-efficacy.
    \item \textbf{\textit {Mixed-race participant pairs benefited from diversity of ideas from their partners:}} Mixed-race participant pairs (green, square trend line) had the lowest average score for question 6 - "improved creativity" (refer to Figure \ref{fig: pp post study}). However, in interviews, mixed-race participants expressed that their partner brought a different perspective for ideas, steps to solve the problem, and how to fix bugs in the code. Five participants from mixed-race pairings noted having different perspectives as a benefit to completing the task with a partner from a different racial group. P12-W1B1 (P12 was a mixed-race pair) discussed the advantages of working with a partner from a different racial group, \textit{“\dots because they see things that you don't see, and you see things that they don't see\dots so communication within [different] people is always a good thing.”} One participant (P8-W1Wh1) stated their preference for having a pair programming partner from a different racial group. When asked about the reasoning for this preference P8-W1Wh1 (P11 was a same-race pair) said, \textit{" I assume, if you had 2 people from different backgrounds, racial or ethnic or otherwise you would potentially have more access to a diverse thought process for problem solving."} A school administrative study described how in order to give students a range of different perspectives and backgrounds to draw from in their educational environment, it is crucial for instructors and staff teams in schools to consist of people from different racial groups~\cite{ngounou2019value}.  
 \end{itemize}
\end{itemize}


\textcolor{blue}{frequencies table or graph of role exchange}

\subsubsection{Role-exchange dynamics} Roles are well-established partner dynamics in pair programming. The primary two roles are driver and navigator. The driver writes the code while the navigator verbally guides with suggestions. The frequency and flexibility of how pairs exchange roles can determine individuals level of engagement in the programming task~\cite{bryant2006pair, zhong2017investigating}.

Participants exchanged roles primarily because they were uncomfortable with the coding syntax. Participants felt at ease as the driver when they had self-confidence through recent experience with Java. P5-M1Wh1 said, \textit{"If I'm confident enough, I would definitely be the driver."} P7-W2Wh2 said, \textit{" If I felt confident with the syntax of the code I was writing."} Participants felt secure as the navigator when they wanted to learn or thought of solutions to solve the problem. P10-M1B1 said, \textit{" If I have a clear idea in my mind on how I want to execute [the task]."} Role-exchange dynamics varied between same- and mixed-race participant pairs.
%P1-M2B2 said, \textit{"When I'm really confident in the code itself I'd like to be the driver."}

\begin{itemize}
\item[] \textbf{Key Findings}
 \begin{itemize}
    \item \textbf{\textit {Navigator of same-race participant pairs tended to disengage from the task:}} Disengagement from the navigator is described as the navigator failing to grasp the task and letting the driver continue with the programming by themselves. The disengaged navigator loses the advantages of pair programming when they stop participating and lack concern in completing the task~\cite{plonka2012disengagement}. Five participants from same-race participant pairs mentioned experiencing partner disengagement or being disengaged from the task. High levels of comfort could be the reason same-race pairs experienced disengagement from the navigator. P1-M1B1 (driver) talked about this phenomenon, in his interview, when asked about how his partnership with P1-M2B2 (navigator) felt, \textit{"I feel like since I was talking so much, I wasn't getting a lot of reciprocation other than just like, yeah, you're right, you can do this..."} P2-M1B1 (the navigator) expressed his disengagement during the task, \textit{“...there [were] definitely times when I was kind of, I didn't know honestly what [was] going on...”} Same-race pairs experiencing navigator disengagement possibly negatively affected productivity and code quality because one partner worked to solve the task alone instead of utilizing the skill set of both partners.
    \item \textbf{\textit {Mixed-race participant pairs explicitly discussed roles:}} All of the mixed-race participant pairs communicated explicitly and strictly adhered to the driver/navigator roles. The mixed-race pairs discussed pair programming roles at the beginning, middle, and end of the interaction. For example, we observed P12 (mixed-race) discuss roles 7 times while P6 and P10 (same-race) discussed roles on average 1 time. All of the mixed-race pairs discussed pair programming at the beginning, middle, and end of the interaction. When asked if the pair assigned roles P9-M2Wh2 said \textit{"We went pretty explicit, I said. Hey, do you want to be a driver? He said. Sure, and he was a driver. I was navigator... I think we stuck pretty close into the roles."} In interviews, we confirmed that same-race pairs lacked explicit discussion of driver/navigator role. When asked about how they decided to switch roles P9-M2Wh2 said \textit{“For the most part we had one person do most of the driving...I did a little bit...I wasn't necessarily navigating [or] driving [so] he did most of the driving and then he was also navigating as well.”} The discussion and use of pair programming roles allowed mixed-race pairs to progress quickly through the task. 
 \end{itemize}
\end{itemize}

\begin{comment}
\subsubsection{Effect of communication medium}
Communication mediums used during pair programming are... How partners ...

\textbf{Key takeaways:}
\begin{itemize}
    \item \textbf{\textit {Participants preferred in-person for learning and interactions:}}
    \item \textbf{\textit {Participants preferred remote for convenience: }} (privacy, can do what I want, easier functionality -share screen)
\end{itemize}
\end{comment}

\begin{tcolorbox}[width=\textwidth,
    colback={black!10},
    %title={RQ3 - Diversity's Double-Edged Sword},
    %colbacktitle=blue!40,
    %coltitle=black
    ]
    \begin{center}
        Diversity had a positive impact on collaboration from sharing decision-making, exchanging pair programming roles and an increased variety of ideas.
    \end{center}
\end{tcolorbox}  
% however, it also had a negative impact due to increased interruptions. 

\subsection{RQ3: What factors contribute to the attitude and dynamics differences between same- and mixed-race participant pairs?}

To explore the influence of individuals' awareness of their partners' racial backgrounds on their attitudes and behaviors, we conducted interviews and examined their perspectives during interactions with individuals from diverse racial backgrounds. Our findings indicated no disparities in trust and empathy but highlighted variations in communication, vulnerability, cultural rapport, comfort levels, and relatability among individuals of different racial backgrounds.

\subsubsection{\textcolor{red}{dont understand title} No disparities due to Racial Awareness}
%To understand the cultural background of programmer pairs influence on communication, rapport-building, comfort level, question-asking, and empathy within the context of pair programming, and how these factors differ between same- and mixed-race participant pairs.

\begin{enumerate}[label={(\arabic*)}, noitemsep]
\item \textbf{Trust and Racial Awareness in Pair Programming Dynamics}

Trust plays a pivotal role in pair programming, as partners rely on each other's advice and contributions. Participants generally placed their trust in partners with experience, higher skill levels, or those they had established relationships with. For instance, P6-M1Wh1 expressed his trust in his partner due to the latter's superior skills, stating, \textit{“I felt like P6-M2Wh2 knew what he was doing a lot \dots he seemed to jump right in and get to it \dots so I was fine with letting him go with his thing\dots I think we have the same general concept of what to do his was just better and more advanced.”} 

\item \textbf{\textcolor{cyan}{Empathy and Racial Awareness in Pair Programming Dynamics} Empathy Toward Minorities}

 While trust in pair programming often correlated with participants' skill levels, an additional layer of caution emerged, shaped by racial awareness during collaborative efforts. P11-W2Wh2 provided valuable insight into this racial awareness, stating, \textit{“I do try to, as I mentioned earlier, especially when working with women or individuals who identify as non-binary, Black, Asian, or from any other racial background [that’s] not White, [I make an effort] to be highly conscious of my words. As someone who identifies as a woman and is also white, I recognize that I possess certain privileges and a degree of authority in such situations. Therefore, I am vigilant not to overstep boundaries and ensure that I provide them with the space to express themselves and discuss the task. [I'm] simply trying to remain acutely aware of the context at hand.”} This heightened racial awareness introduced nuances in attitudes and dynamics, particularly evident in interactions involving both same- and mixed-race participant pairs.


\end{enumerate}

\subsubsection{\textcolor{red}{dont understand title} Disparities among Races}
%Trust is a key dynamic of pair programming because partners must take each other's advice and contribution into consideration. All participants trusted a partner with experience, a higher skill level, or after building a relationship. P6-M1Wh1 mentioned that he trusted his partner because of his higher skill level, \textit{“I felt like P6-M2Wh2 knew what he was doing a lot \dots he seemed to jump right in and get to it \dots so I was fine with letting him go with his thing\dots I think we have the same general concept of what to do his was just better and more advanced.} Although participants mainly attributed trust to skill level, they exercised caution through racial awareness during the task. P11-W2Wh2 explained this racial awareness, \textit{“I do try to like I said previously, especially with women or people who identify as non-binary and either Black or Asian or any other race [that’s] not White, [I try to] be very cognizant of what I'm saying because while I'm also someone who identifies as a woman, I'm also white. So I do have some privilege and somewhat authority in the situation. So being cognizant of that and not overstepping and making sure I give them the space to be themselves and also communicate about the problem. [I'm] just trying to be more aware of the situation at hand.”} Racial awareness causes differences in attitude and dynamics amongst same- and mixed-race participant pairs  

%\item \textbf{\textit {Participants trusted partner after building relationship:}} interview codes , if you worked with them before, man/woman example - haven't build more relationship with woman

%In the retrospective interviews, 7 participants stated a preference for a partner from the same-racial group, 11 participants stated no preference and 1 participant preferred a different racial group.

\begin{comment}
\begin{itemize}
\item[] \textbf{Key Findings}
 \begin{itemize}
  \item Item 1
  \item Item 2
  \item Item 3
 \end{itemize}
\end{itemize}
\end{comment}

\begin{enumerate}[label={(\arabic*)}, noitemsep]
  %  \item \textbf{\textit{Same-race participant pairs communicated better while mixed-race participant pairs lacked communication:}} 

 \item \textbf{\textit{Communication Disparities in Same- and Mixed-Race Participant Pairs:}} 
Effective communication is a multifaceted skill encompassing active listening, clear articulation of ideas, open sharing of thoughts, and the cultivation of approachability. It is noteworthy that a survey conducted among professional developers at Microsoft identified good communication as one of the top ten qualities desirable in a pair programming partner~\cite{begel2008pair}. Within the realm of pair programming, the dynamics of communication underwent distinct influences driven by racial awareness, particularly evident within same-race and mixed-race participant pairs.

Same-race participant pairs often exhibited superior communication, an outcome often linked to the heightened comfort levels stemming from shared demographics. P2-M1B1 underscored this aspect, emphasizing that a deeper sense of comfort facilitated open and effective communication with partners. He stated, \textit{“I do prefer partnering with individuals from the same demographic or racial background because it often leads to smoother communication. We tend to find it easier to convey certain ideas or share similar viewpoints due to our shared experiences.”}

Conversely, mixed-race pairs frequently encountered communication challenges stemming from concerns about inadvertently causing offense or misunderstanding due to racial dynamics. P11-W2Wh2, a participant in a mixed-race pair, candidly expressed how race considerations occasionally hindered their ability to communicate openly. She noted, \textit{“...it would be naive to deny the impact of race on our communication. There were instances where I hesitated to fully express myself out of fear that it might be perceived as overstepping boundaries.”}

These contrasting communication dynamics between same-race and mixed-race participant pairs presented distinct challenges for the latter, emphasizing the pressing need to address and navigate such issues to optimize pair programming interactions.
    
    
    
    %Listening, expressing ideas clearly, voicing inner thoughts, and being approachable are all aspects of communication. A survey amongst professional developers at Microsoft found that good communication was among the top ten qualities for a pair programmer partner~\cite{begel2008pair}. Racial awareness affected the communication dynamics between same- and mixed-race participant pairs. Better communication between same-race pairs is possibly because of higher comfort levels. P2-M1B1 affirmed that a higher comfort level led to open communication with his partner, \textit{“I do like partnering [with] people who are the same demographic or same race, just because [I] may just be able to like, communicate certain things or you know, we might just have similar ideas just because of similar experiences.”} Due to hesitation of being inconsiderate of their partner, mixed-race pairs often lacked communication. P11-W2Wh2 (P3 was a mixed-race pair) expressed how race decreased communication within their partnership, \textit{“\dots like it would be naive to say no [that race didn't affect communication]. I even felt like there were times where I didn't fully communicate [because] it could have came across like I was overstepping\dots"} Mixed-race pairs lacked communication which caused a hindrance to pair dynamics. 
    \item \textbf{\textit {Same-race participant pairs were vulnerable with each other and mixed-race participant pairs showed empathy towards their partner:}} 

    
%\item \textbf{\textit {Same-race participant pairs were vulnerable with each other and mixed-race participant pairs showed empathy towards their partner:}}

Vulnerability, characterized by participants opening up and sharing personal aspects of their personality with their partner~\cite{schroeder2009vulnerability}, manifested differently within same-race and mixed-race participant pairs.

In the case of same-race pairs, vulnerability was more pronounced as participants felt a sense of camaraderie rooted in shared experiences. P4-W1B1, part of a same-race pair, described this vulnerability, stating, \textit{“It's more just like we've all been through the same stuff like we're just trying to get this done. So let's just try to knock this out, and there's more of a jovial tone\dots probably from the same [racial group]. I feel like there's maybe just greater ease, and I could reveal all of my personality\dots”}

Conversely, mixed-race participant pairs demonstrated empathy towards each other, marked by heightened awareness and consideration of their partner's feelings and reactions. \textcolor{red}{Always use numbers...in this section use numbers} Several participants in mixed-race pairs mentioned exercising extra caution when working with partners from different racial backgrounds. For instance, P11-W2Wh2 (P11 was part of a mixed-race pair) expressed the need for heightened sensitivity, explaining, \textit{"Yeah, you sort of [have to be] more careful about what you [say] just because, like [I] said, especially when it comes to people who are already in marginalized groups\dots"}

This empathy and carefulness exhibited by mixed-race pairs can be reminiscent of findings from a counseling psychology study on mixed-race counselor/client dynamics, which highlighted how counselors' culturally-sensitive or culturally-blind responses can significantly influence clients' reactions and engagement in counseling sessions~\cite{pomales1986effects}.
    
    
    %Vulnerability is when participants expose or open up personal aspects of their personality to their partner~\cite{schroeder2009vulnerability}. Same-race participant pairs were vulnerable with each other while working on the task. P4-W1B1 spoke about the vulnerability she experienced (P4 was a same-race pair), \textit{“It's more just like we've all been through the same stuff like we're just trying to get this done. So let's just try to knock this out and there's more of a jovial tone\dots probably from the same [racial group]. I feel like there's maybe just great, better ease or I could reveal all of my personality\dots”} Mixed-race participant pairs showed each other empathy by being extra careful of their actions towards their partner. Three participants stated that they exercised extra carefulness when working with their partner from a different racial group. Regarding collaborating with her partner, P11-W2Wh2 (P3 was a mixed-race pair) said, \textit{"Yeah, you sort of [have to be] more careful about what you [say] just because, like [I] said, especially when it comes to people who are already in marginalized groups\dots"} A past counseling psychology study on mixed-race counselor/client dynamics found that a counselors culturally-sensitive or culturally-blind responses can influence a clients reactions and engagement in the session~\cite{pomales1986effects}. 
    
    \item \textbf{\textit {Same-race participant pairs had a cultural rapport but lacked experience with other cultures:}} 
    The concept of cultural rapport, often characterized by an unspoken understanding, familiarity with culturally specific terms, and the exchange of non-verbal cues~\cite{johnson1999ties, merriam2001power}, played a significant role in shaping interactions within same-race participant pairs. These pairs tended to share a natural cultural rapport with their partners, which translated into increased comfort levels during collaboration. P3-W1B1 articulated this phenomenon, explaining, \textit{“\dots I think in general, I do find it easier to work in groups or collaborate with other people from [the] same racial or ethnic background just because there's some stuff that you sort of get, even if it's like stuff that's not directly related to the task. Building cultural rapport with somebody does go a long way in making you feel more comfortable and able to do the task that you're working on\dots”}

Conversely, participants frequently noted their lack of experience when it came to pair programming with individuals from different racial backgrounds. This lack of exposure often resulted in uncomfortable situations. For instance, P1-M1B1 admitted to his limited experience collaborating with individuals from different racial groups, stating, \textit{"I grew up like in Black areas only I always went to all Black schools, everything so like there would just be like a level of uneasiness working with different races."} Similarly, P9-M2Wh2 recounted a personal anecdote highlighting the impact of limited cross-cultural exposure, sharing, \textit{"For example, when I was young I did not encounter Black people at all right until college started\dots I guess here's [a] good anecdote. I remember when I first became a TA, I associated lynching (the unauthorized public hangings of Black people in the US from the 1890s to 1940s ~\cite{wood2011lynching}) with like werewolves right? It's from a game I would play. I was telling a professor I have a really good joke\dots I don't remember the full context. I think I was just going to make fun of [a college] team [by writing] oh, don't lynch me for this! But then [the professor] was like you may not want to use that word. I'm like, oh, I didn't think of this."}

Despite their lack of experience with individuals from different cultures, same-race participant pairs often displayed a strong cultural bond, emphasizing the importance of these cultural affinities in fostering comfort and rapport among collaborators.
    
    
    
    %Cultural rapport or 'insider' perspective is a unspoken understanding or culturally specific terms that could be understood without translation, and non-verbalized responses expressed through non-verbal cues~\cite{johnson1999ties, merriam2001power}. Same-race participant pairs had a natural cultural rapport with their partners leading to increased comfort levels. P3-W1B1 affirmed this observation, \textit{“\dots I think in general, I do find it easier to work in groups or collaborate with like other people from [the] same racial or ethnic background just because there's some stuff that you like you sort of get, even if it's like stuff that's not directly related to the task. Building a cultural rapport with somebody does go a long way in making you feel more comfortable and able to do the task that you're working on\dots”} Several participants stated that they have no experience pair programming with a partner from a different racial group. Participants mentioned how their lack of experience with other cultures causes uncomfortable situations. P1-M1B1 spoke on his lack of experience working with different racial groups, \textit{"I grew up like in Black areas only I always went to all Black schools, everything so like there would just be like a level of like uneasiness working with different races."} P9-M2Wh2 recalled a personal story where lack of exposure put him in an awkward situation with a classmate \textit{" For example, when I was young I did not encounter Black people at all right until college started\dots I guess here's [a] good anecdote. I remember when I first become a TA I associated lynching (the unauthorized public hangings of Black people in the US from the 1890s to 1940s ~\cite{wood2011lynching}) with like werewolves right? It's from a game I would play. I was telling a professor I have a really good joke\dots I don't remember the full context. I think I was just going to make fun of [a college] team [by writing] oh, don't lynch me for this! But then [the professor] was like you may not want to use that word. I'm like, oh, I didn't think of this."} Although they lacked experience with other cultures, same-race participant pairs showed a strong cultural bond. 
    
    \item \textbf{\textit {Participants felt comfortable working with same-race individuals but had anxiety working with other races:}} 
    
    The concept of comfort levels, often associated with the "feel-good" effect in collaborations, pertains to the extent to which both partners feel at ease during their interactions and how this comfort can potentially influence their performance~\cite{muller2004empirical}. Seven participants in this study highlighted the advantages of working with individuals of the same racial background, emphasizing the higher level of comfort and the sense of natural connection they experienced. P3-W1B1 (P3 was a same-race pair) articulated her reasons for feeling more at ease during the task, stating, \textit{“\dots I will say there could have just been some natural comfort being with someone [I'm] slightly more familiar with\dots I think that could have maybe unknowingly affected how I talked, how I joked, or you know things of that nature. I think there's benefit in me, being not as nervous, or on edge, or trying to present a certain way, I was able to be myself more likely.”}

Anxiety, particularly in the workplace, can lead to fatigue, reduced focus, and decreased overall performance~\cite{haslam2005anxiety}. While many software companies have recognized the importance of supporting mental health programs, including Employee Assistance Programs (EAPs), Mental Health Benefits, and Mental Health Training, the issue of anxiety continues to affect employees. The availability of tailored mental health programs and resources for employees can vary significantly from one company to another. Some companies proactively acknowledge the significance of addressing the mental health needs of their diverse workforce and may offer specific programs or initiatives to support employees from marginalized groups. However, not all companies provide these resources, and the extent of support can differ based on factors such as the company's size, industry, and commitment to diversity and inclusion.

Four participants in this study specifically pointed out discomfort and anxiety as drawbacks that had a detrimental impact on their productivity in the workplace. P1-M1B1 shared his experiences of anxiety while working with individuals from different racial backgrounds, explaining, \textit{"\dots I don't have that much exposure to working with someone that's not Black so it'd be like some anxiety from just getting used to that format."}

In the realm of psychology, research on same-race Black therapeutic pairs has found that the implicit degree of comfort naturally present, combined with the use of culturally based vernacular, can facilitate the rapid development of bonds~\cite{goode2016unspoken, cabral2011racial}.
    
    %Comfort levels, also known as the "feel-good" effect describes how comfortable both partners feel during the interaction which might affect their performance~\cite{muller2004empirical}. Seven participants highlighted a higher level of comfort and a natural connection as benefits to working with same-race individuals. P3-W1B1 (P6 was a same-race pair) explained her reason for a higher comfort level during the task, \textit{“\dots I will say there could have just been some natural comfort being with someone [I'm] slightly more familiar with\dots I think that could have maybe unknowingly affected how I talked, how I joked, or you know things of that nature. I think there's benefit in me, being not as nervous, or on edge, or trying to present a certain way, I was able to be myself more likely.”} Anxiety, at the workplace, can cause tiredness, lack of focus and decreased performance~\cite{haslam2005anxiety}. While many software companies have recognized the significance of supporting mental health programs, including Employee Assistance Programs (EAPs), Mental Health Benefits, and Mental Health Training, the issue of anxiety persists among employees. In the workplace, the availability of tailored mental health programs and resources for employees can vary widely from one company to another. Some companies are proactive in recognizing the importance of addressing the mental health needs of their diverse workforce and may offer specific programs or initiatives to support employees from marginalized groups. However, not all companies provide these resources, and the extent of support can differ based on factors such as the company's size, industry, and commitment to diversity and inclusion. Four participants highlighted levels of discomfort and anxiety as drawbacks that had a negative impact on their productivity at the workplace. P1-M1B1 spoke on anxiety he has experienced working with other races, \textit{"\dots I don't have that much exposure of working with someone that's not Black so it'd be like some anxiety from just getting used to that format."} Psychology literature on same-race Black therapeutic dyads discovered that because of the implicit degree of comfort that is naturally present and the usage of culturally based vernacular it is easier and faster to develop bonds~\cite{goode2016unspoken, cabral2011racial}.
    
    \item \textbf{\textit {Participants related more to same-race individuals but "sugar coat" when working with other races:}} 
    
    Relatability, an attribute characterized by simplicity in comprehension and the ability to empathize with others~\cite{aish2018people}, played a role in how participants expressed uncertainty during collaborative tasks. Participants often demonstrated uncertainty by conveying incomplete thoughts or statements or by explicitly expressing confusion about code bugs or Java programming syntax. For instance, P4-W1B1 inquired of P4-W2B2, \textit{"What's that?"} in reference to \verb|Scanner in = new Scanner(System.in);| within the code. P4-W2B2 responded, \textit{"I don't know what that means. I'm going to look it up. I'm going to look up the scanner."}

Notably, same-race participant pairs exhibited a \textcolor{red}{how much higher?}higher frequency of uncertainty expression compared to mixed-race participant pairs. This pattern may be attributed to the greater comfort levels experienced when collaborating with individuals of the same racial background. P3-W1B1 (P3 was a same-race pair) spoke about openly acknowledging uncertainty with her partner at the outset of the task, stating, \textit{"I probably knew that I was going to take on that driver role a little bit more since we both expressed uncertainty\dots"}

Participants also discussed a tendency to employ indirect communication, often referred to as "sugar coating"~\cite{sices2009sugar}, when collaborating with individuals from different racial backgrounds. P2-M1B1 elaborated on this phenomenon, explaining, \textit{"\dots someone who's similar to me demographically\dots I think it would just be a lot faster because I could be super open with them, super transparent. I wouldn't have to sugar coat anything. I could just say, 'Hey, I'm having this problem, and I don't know what to do,' and they could really level with me and relate to me\dots"}

While participants tended to identify more with individuals of the same racial background, they often moderated their communication style when collaborating with individuals from different racial backgrounds, highlighting the complex interplay between relatability, comfort, and communication dynamics in collaborative settings.
    
    %Relatable is an attribute defined as being simple to comprehend or sympathetic toward others~\cite{aish2018people}. Participants were relatable when expressing uncertainty during the task. Participants showed uncertainty by saying unfinished ideas/statements or explicitly expressing confusion about code bugs or Java programming syntax. For example, P4-W1B1 asked P4-W2B2, \textit{"Whats that?"} referring to \verb|Scanner in = new Scanner(System.in);| in the code. P4-W2B2 responded, \textit{"I don't know what that means. I'm go look it up. I'm going to look up the scanner."} Same-race participant pairs had higher accounts of uncertainty than mixed-race participant pairs. This may correlate to higher comfort levels when working with same-race individuals. P3-W1B1 (P6 was a same-race pair) talked about explicitly expressing uncertainty with her partner during the beginning of the task, \textit{"I probably knew that I was gonna gravitate [to] that driver role a little bit more since we both expressed uncertainty\dots"} Participants mentioned how they "sugar coat" (indirectly communicate~\cite{sices2009sugar}) when working with other races. P2-M1B1 talked about this phenomenon, \textit{"\dots someone who's similar to me like demographics\dots I think it would just be a lot faster just because I could be super open with them super transparent. I don't have to sugar coat anything I'm just like, hey I'm having this problem [and] I don't know what to do [and] they could really level with me [and] really relate to me\dots"} Participants tended to identify more with same-race individuals, but softened their vernacular when working with other races.
\end{enumerate} 

\begin{tcolorbox}[width=\textwidth,
    colback={black!10},
    %title={RQ3 - Diversity's Double-Edged Sword},
    %colbacktitle=blue!40,
    %coltitle=black
    ]
    \begin{center}
        Diversity had a negative impact on pairs attitude \& dynamics due to lack of communication, heightened anxiety, and empty conversational shifts. 
    \end{center}
\end{tcolorbox}  

    % Partners being sensitive to each other (i.e., taking turns talking, listening to ideas) can increase the pairs performance~\cite{roschelle1995construction}.
    
    %Many coding bootcamps and coding schools (Code2040 \cite{}, Black Girls CODE \cite{}) as well as universities (Historically Black Colleges and Universities (HBCUs)\cite{})  in the United States are committed to promoting diversity and inclusion, and they actively work to support underrepresented groups, including Black individuals, in tech education.  But these sometimes do not give them exposure to other races...

    %Two Black participants from mixed-race pairings noted high comfort levels as a benefit from previous work experiences during collaboration with a partner from the same racial group during the retrospective interviews.


    %The lack of diversity in tech companies can contribute to a hostile or unwelcoming work environment for Black employees, leading to higher turnover rates and reduced job satisfaction.

    %In general, same-race White pairs and mixed-race pairs had lower uncertainty instances which may suggest discomfort expressing confusion to their partner.
    
    %\item \textbf{\textit {Vulnerable with same race pairs while mixed-race showed more empthay with extra careful with other races}} 
    %vulnerable-more open, asked more questions, uncertanity

    %In general, same-race White pairs and mixed-race pairs had lower uncertainty instances which may suggest discomfort expressing confusion to their partner.

    %When asked if race had any impact on the Main Task collaboration P11-W2Wh2 said, \textit{“...I think it would also be like a disservice to [her] if I immediately flat out said no, because like, I think her opinion in the situation is like what is more meaningful...”}


    %P4-W1B1 also commented on past work experiences, \textit{"...I feel like [when] working with black students they don't see me that way and so I feel more okay to be like, hey can we do this, let's try this without like fear of retribution."}


   % P1-M2B2 expressed how he was comfortable communicating with his partner \textit{“...I would enjoy it more with someone of the same race. But if it was a different race it'd be no issue in completing the task...some of the words we were using it just rolls off the tongue that you really couldn't use with a different person from a different race. So when P1-M1B1 would say all right, I'm gonna do that. I automatically understood it like, okay, he's going to do that [and] I'm going to do it like this...I've worked with dozens of [people] I don't [look] like before, and it's great [but] you have to kind of change the way you talk for them to fully understand...It works better when you're working with a person within the same race as you [because] it felt more comfortable that way.”} 


